Programmable Dataflows: Abstraction and Programming Model for Data Sharing

Data sharing is central to a wide variety of applications such as fraud detection, ad matching, and research. The lack of data sharing abstractions makes the solution to each data sharing problem bespoke and cost-intensive, hampering value generation. In this paper, we first introduce a data sharing model to represent every data sharing problem with a sequence of dataflows. From the model, we distill an abstraction, the contract, which agents use to communicate the intent of a dataflow and evaluate its consequences, before the dataflow takes place. This helps agents move towards a common sharing goal without violating any regulatory and privacy constraints. Then, we design and implement the contract programming model (CPM), which allows agents to program data sharing applications catered to each problem's needs. Contracts permit data sharing, but their interactive nature may introduce inefficiencies. To mitigate those inefficiencies, we extend the CPM so that it can save intermediate outputs of dataflows, and skip computation if a dataflow tries to access data that it does not have access to. In our evaluation, we show that 1) the contract abstraction is general enough to represent a wide range of sharing problems, 2) we can write programs for complex data sharing problems and exhibit qualitative improvements over other alternate technologies, and 3) quantitatively, our optimizations make sharing programs written with the CPM efficient.

==> old/bootstrappingtrust.tex <==
\section{Bootstrappping Trust}
\label{sec:bootstrappingtrust}


What to do other than rely on enclave?

How do we know who's "Steven"?

Who can and who should see all of the functions on DS?

Trust from Zero

There are so many layers of trust. For example, in MPC you must trust the math is correct, then you must trust the implementation. What do you trust here?

Trust Built from Zero-Knowledge-Proof?

==> old/escrow_old.tex <==
\section{Data Sharing System}

\notera{i dont know where this is going, and it does not tell me anything about what this section is about (which is the main goal)}

For any data sharing process, a number of these scenarios can occur. Example \ref{ex:example} is composed of Single-source, Preconditional and Multi-source, Preconditional scenarios. There are existing solutions to some these individual scenarios, but this means that multiple individual solutions must be chained together to accomplish a data sharing process. This induces technical overheads, platform and data migration costs, and an expanding trust domain for each additional solution. There lacks a unified system that has the flexibility to execute all of these scenarios to ultimately achieve a goal state.
% In this section we first present an overview of our unified system to achieve goal states in the data sharing process in Section \ref{subsec:overview}. We then present our solution to support the heterogeneity of sharing scenarios in Section \ref{subsec:epf}. We then describe how we execute shares while preventing unapproved transitions in Section \ref{subsec:unapprovedt}.


% We now present Data Station, a system that implements the details necessary to support the Sharing API to support the \textit{entire} data sharing process. An overview of Data Station is shown in Figure \ref{fig:overview}, which shows how agents deploy and use the system in practice.

% \steven{there’s no order or logic in why these are the things that have to happen. You could start by enumerating and justifying what must happen. Then explain very briefly each step and how it relates to each other}

% % Rather than allowing any direct API calls, agents instead call functions that are a \textit{customized} layer that is built atop of the Sharing API that can be tailored to a specific scenario's needs. These functions include custom-written logic before registering data elements, suggesting and approving shares, or running a SQL query or training a machine learning model on some data elements. These functions are initially uploaded to a Data Station instance as it launches on a server. Agents register themselves with Data Station (\textit{register\_agent()}). They first show themselves the uploaded functions with \textit{show\_function()}; then they call the function with \textit{call\_function()}. In Figure \ref{fig:overview}, agent 1 sees that the callable functions include \textit{upload\_de()}, \textit{suggest\_share()} and so on. Agent 2 uploads a data element to Data Station by calling \textit{call\_api()}, and passing in the name of the function, \textit{upload\_de}, and any other additional parameters, and gets a success message from the server. From this point, the agents can continue to suggest, approve, and execute shares.

% % Agents call the following API endpoints from some interface: register\_agent, show\_function, or call\_function.
% % \begin{myitemize}
% %     \item \mypar{register\_agent()} Agents use this API to register themselves, by specifying a username and password.
% %     \item \mypar{show\_function()} Agents use this to show all functions that they can call.
% %     \item \mypar{call\_function()} Agents use this to call the available functions.
% % \end{myitemize}

% At time 0, a a Data Station instance is launched on a server, which includes a list of functions that users can call, like registering data elements, suggesting and approving shares, or running a SQL query or training a machine learning model on some data elements. To use these functionalities, agents interact with the Data Station instance on the server by calling the following API endpoints from some interface: register\_agent, show\_function, or call\_function.
% \begin{myitemize}
%     \item \mypar{register\_agent()} Agents use this API to register themselves, by specifying a username and password.
%     \item \mypar{show\_function()} Agents use this to show all functions that they can call.
%     \item \mypar{call\_function()} Agents use this to call the available functions.
% \end{myitemize}

% Once the agent has registered themselves, they first look at what functions are available through \textit{show\_function()}, then actually call these functions through \textit{call\_function()}. In Figure \ref{fig:overview}, agent 1 sees that the callable functions include \textit{upload\_de()}, \textit{suggest\_share()} and so on. Agent 2 uploads a data element to Data Station by calling \textit{call\_api()}, and passing in the name of the function, \textit{upload\_de}, and any other additional parameters, and got a success message from the server. From this point, the agents can continue to suggest, approve, and execute shares.

\subsection{System Overview and Requirements}
\label{subsec:overview}

\begin{figure}%
    \centering
    \includegraphics[width=\columnwidth]{figures/ds_overview.png}
    \caption{Data Station Overview}%
    \label{fig:overview}%
\end{figure}

\notera{this is repetitive (it's been already said before)}

As we describe in the previous sections, data sharing is a process, composed of a series of sharing scenarios that represent transitions toward the goal state. Each step towards the goal state is unique to the process, and to facilitate these scenarios, we present Data Station, a system which supports an \textit{entire} data sharing process, from an initial state to a goal state, by implementing the details necessary to execute a wide range of scenarios through the Sharing API. An overview of Data Station is shown in Figure \ref{fig:overview}.

We start with an agent that would like to commence a data sharing process. \notera{so the agent deploying DS needs to write the program?}They deploy an instance of Data Station with a customized set of functions that is built atop of the Sharing API. These functions are tailored to the scenarios of the particular process, with custom-written logic that occurs before the Sharing API registers data elements or suggests and approves shares. The logic for $f$ on data, such as executing a SQL query or training a machine learning model on some data elements, is customized to the scenario as well. \notera{any agents?}Any agents interested in participating within this process first register themselves \notera{how do they discover the instance? how do they know this is the instance they think?} with this instance Data Station (\textit{register\_agent()}). They can now see the custom-written functions with \textit{show\_function()}; they then call one of these functions with \textit{call\_function()}.

\notera{why is the workflow above good? if i'm not convinced is good I won't care about what's needed to support it. These requirements, furthermore are not only good for that workflow but many others. So they should be introduced after those workflows are clear to the reader}
To support this workflow, we enumerate the following requirements for a system whose goal is to facilitate an entire process of data sharing.

\notera{name these requirements (R1, R2, ...) so you can refer to them throughout the section and explain how you address them}

\begin{myenumerate}
    \item \textbf{Support the suggestion and approval of any number of shares, for a wide range of possible shares.} \notera{implement the share abstraction} Multiple shares may need to \notera{multiple shares, always?}be created and executed in a data sharing process. The system needs to allow agents to suggest and approve any number of shares. Moreover, agents may want to execute shares with arbitrary functions and constraints. The system should be flexible enough to support any specifications of the agents, data elements, and functions that define a share. 
    \item \textbf{Support the execution of suggested shares.} In additional to allowing agents to specify the shares, the system should provide mechanisms to actually execute the shares, i.e. computing $f(P)$. \notera{vague}
    \item \textbf{Ensure that no unexpected transition ever occurs unless agents have specified it through a share.} \notera{what is unexepcted if not a transition that agents did not approve through the share?} Examples of unexpected transitions can include an attacker gaining access to data that is stored on disk, or data in-memory during the execution of share. \notera{what else?}
    \item \textbf{Meet all requirements above efficiently.} Without reasonable runtime, executing numerous shares to work towards $GS$ would be impractical. \notera{what does impractical mean?}
\end{myenumerate}

As far as we know, Data Station is the first system designed to satisfy all of the above requirements, hence enabling data sharing. We first explain how our system works with the heterogeneity of sharing scenarios in Section \ref{subsec:epf}, thus addressing requirement 1. We then explain how shares are actually executed, as well as the security guarantees behind executing shares in Section \ref{subsec:unapprovedt}, thus addressing requirement 2 and 3. Lastly, the efficiency of our system is evaluated in Section \ref{sec:evaluation}.

\subsection{Escrow API and Escrow Programming Framework} 
\label{subsec:epf}

\notera{paragraph is too long and too windy. go to the point and make it crisp. this is about letting any sharing application be written over the escrow}
In Figure \ref{fig:overview}, we explained \notera{where was this explained} that at time 0, a Data Station instance is launched on a server, including a list of functionalities that users can access. 
% These functionalities allow agents to suggest, approve, and execute shares. 
Data Station provides a native set of APIs for some of these functionalities, called the Escrow APIs. The Escrow APIs includes generic functionalities that are necessary for almost any data sharing scenario, such as registering data elements or suggesting shares. Yet, for any particular data sharing scenario, agents may want to have access to a set of functionalities that are tailored to their needs. For example, they may want automatically add some specific agents to any share that will be created (e.g. an auditor), or require that only data element that are in CSV files can be registered, for easier integration of data elements. Some agents may
want to share the original data elements, while some agents may only want to share aggregate statistics. The idiosyncrasies of the set of functionalities each data sharing scenario requires are handled by an Escrow Programming Framework (EPF) program. We now go into the details of the Escrow APIs and the EPF programs.

\notera{by the time i get here i don't actually yet know why I'm being presented with an escrow API and EPF (which i still don't know what it is)}

\subsubsection{Escrow APIs}

\notera{high-level 1) i lack a justification for why these APIs are all what we need 2) the API explanation is informal and driven via examples. it should instead be technical, top-botton, and examples after the explanation}

The Escrow APIs includes the following APIs that are designed to support the share abstraction.

\notera{this can be explained at a more high-level first, giving the key idea. Then examples can be used to illustrate the API. it's also too long}

\myparnoperiod{register\_data\_element()} Similar to \textit{register\_data\_element()} in the sharing APIs, \notera{what is register-data-element of sharing API? why do we need 2? and why does share need register-data-element? that seems wrong} this API registers a data element with the Data Station. Every data element is assigned a unique ID. As explained in Section \ref{sec:model}, data elements can be stored in a wide range of formats and granularity. One challenge for a system to support the share abstraction is to handle the heterogeneity of data elements. To address this, Data Station requires two attributes from a data element when it is registered: \textit{type} and \textit{access\_parameters}. For example, a relational table stored in CSV can have type "csv", and access\_parameter being the name of the file. A relational table stored on some open data repository can have type "open data", and access\_parameter being a JSON object containing the API key and endpoint from which the data can be retrieved. These two parameters allows functions to customizably access heterogeneous data elements, which we will explain more when we talk about the EPF programs.

\myparnoperiod{upload\_data\_element()} Data Station supports agents uploading their data elements to the station. 

\myparnoperiod{list\_discoverable\_des()} In addition to specifying \textit{type} and \textit{access\_parameters}, agents also specify whether a data element is \textit{discoverable} when they register a data elmement. In some cases, destination agents do not know a priori which data elements help them achieve their goal. Yet, when a share is specified, it needs to include the complete set of data elements $P$ that it will access. On the other hand, source agents may want their data elements be included by shares suggested by other agents, because they believe that their data elements can be helpful for other agents achieving their goals. This API allows agents to see the ids of all discoverable data elements, so that they can include these data elements when suggesting shares, without even knowing a priori the existence of those data elements.

\myparnoperiod{suggest\_share(), show\_share(), approve\_share()} These APIs are implemented as described in Section \ref{sec:share}. Note that when agents suggest a share in Data Station, Data Station automatically populates all source agents as part of $A_{\text{ack}}$, and agents can add additional approval agents if they desire.

\myparnoperiod{get\_all\_accessible\_de(), get\_de\_by\_id()} These APIs are used to access data elements within a template. The first one returns all data elements in $P$, and the second one returns a single data element specified by an ID, if the data element is in $P$.

\notera{this is repetitive again. does not add anything new}
Escrow APIs provides agents with some default functionalities to manipulate shares, which are general enough to be applicable to any data sharing scenarios. Yet, as we have explained, for a particular data sharing scenario, it would be helpful to give agents customized control over the the exact details of these functionalities. We now explain the EPF program.

\notechz{Have a paragraph explaining what happens to registered data elements and shares}

% \mypar{Shares} With the support for agents, data elements, and functions through templates, Data Station can now support shares. We implement the logic of a share in close accordance to Section \ref{sec:share}. A share on Data Station is hence a set of 
% \[\langle A_{\text{dest}}, P, \text{template},\text{parameters}, A_{\text{ack}} \rangle\]

% that can be suggested, viewed, approved, and executed by agents.

% \mypar{Policies} For a destination agent to execute a share and get results, all approval agents must first have set $M() = 1$. Data Station represents $M$ with \textit{policies}. A policy is a triple of $\langle$approval agent id, share id, status = $\{0,1 \}\rangle$. When a new share is suggested, a policy is created for every approval agent for the share. Initially, all policies have status $0$, representing $M() = 0$. An approval agents approving a share sets the status of the corresponding policy to 1. Once all polices for a share has status 1, the share can be executed.

\subsubsection{Escrow Programming Framework}

\notera{top-bottom explanation 1) what is this 2) why we want this 3) how do programs look like 4) what kinds of programs can be written. and then 1) who writes these programs 2) what is new that they need to know (escrow API, etc) ... Once I know what these are, then I may care about template functions. Otherwise, that'll just confuse me since I don't know yet what we are trying to do here. Also, include a figure to illustrate this. Could be shared with section 5}

An EPF program is a program acting as a customizable layer built on top of the Escrow API, written by a developer for any particular instance of Data Station. Upon launching of a specific Data Station instance, Data Station loads an EPF program, which consists of a set of developer-written \textbf{Function API Endpoints}. Rather than allowing calls to the Escrow API directly, Data Station instead has agents call the Function API Endpoints specified within the EPF, and these Function API Endpoints contain the specifications of functionalities that agents can access, for any particular instance of Data Station.

Essentially, the EPF is a collection of functions, written in a high-level language such as Python. These functions can be tagged with two types of decorators: @non\_template, and @template. Any function with any of these tags is a Function API Endpoint, and is callable to an agent. In an EPF, a non-template function is used to manage data elements and shares, and do not need access to data elements. A template functions correspond to the actual $f$ that agents want to run, and requires access to data elements.

\mypar{Non-template Functions} Agents manage shares and data elements using non-template functions. Developers write these functions to customize what Escrow APIs are callable and how they can be called. This gives developers full control over how shares are created and how data elements are registered or uploaded. For example, a non-template function that automatically adds a specific agent to any share created on some Data Station instance, called \textit{suggest\_share\_custom()}, can be implemented by making a call to the \textit{suggest\_share()} provided by the Escrow API, and always add the specific agent ID to the list of approving agents. 

There are numerous use cases for this customized logic:

\begin{myitemize}
    \item Automatically adding an agent, such as an auditor, to $A_{\text{ack}}$ whenever a share is suggested.
    \item Preventing certain kinds of files from being registered.
    \item Converting a file into a specific format before it is uploaded.
    \item Suggesting multiple shares at a time.
    \item Automatically creating, then approving, shares.
\end{myitemize}

\mypar{Templates Functions} To represent $f$ in shares, Data Station uses \textit{template functions}. A template function is any function, written in a high-level language (e.g. Python), that can be parameterized. It can also make calls to any packages available to the high-level language (e.g. numpy, pandas, duckdb, etc.). A template and its specific parameters constitute $f$ in our model. That is, 
\[f(P) \text{ [in the model]}= \text{template}(\text{parameters},P) \text{ [in Data Station]}\]

Because a template function is written in an established high-level language, it provides high usability for the agents when defining functions, as they do not need to learn a new language, or a new set of primitives. A template function also provides full customizability to express a set of functions that can be created from changing parameters. Consider an agent $a_1$ who wants to access a sample of $a_2$'s data element. Without using a template, $a_1$ needs to hardcode the size of the sample into $f$ when specifying the share, say 5 rows. If $a_2$ does not approve this share, $a_1$ either modifies the code of the original function, or needs to write a new function, which limits usability. Specifying functions in shares by parameterizing templates encompasses both the restrictiveness of $f$ in the model sense, which represents the \textbf{exact} computation to run on data elements, and the ease of specifying a wider range of $f$ by changing the parameters.

When suggesting a new share, agent will refer to a particular template function, along with its parameters. Agents can then execute this share, to call this template function with parameters given by the share, once the share is approved (otherwise, the share does not execute). Since template functions access data elements, they make calls to \textit{get\_all\_accessible\_des()} or \textit{get\_de\_by\_id()}, provided by the Escrow API. These data elements may have been registered as different types, and it is up to the developer to write code to support each type, based on their access\_parameters.

Lastly, functions not tagged with either decorators act as helper functions, which can be called by other functions in the EPF.

\subsection{Executing Shares While Preventing Unapproved Transitions}
\label{subsec:unapprovedt}

A data sharing system not only needs to allow agents to suggest a wide range of possible shares, but also needs to be able to execute the shares, that is, computing $f(P)$. This is a non-trivial task when $P$ involves multiple source agents, given agents' various constraints. We first discuss one baseline for executing arbitrary shares: delegate the computation to a \textbf{trusted third party}.

\mypar{Baseline: Trusted Third Party} Consider how the \notera{outdated}three labs in Example \ref{ex:example} can actually calculate the aggregate statistics of their joint data. One way is for the labs to find a trusted third party and each send their data to it. The trusted third party will calculate the statistics, check that the statistics fall within the accepted range, and release to the researcher. 

Using a third party can execute any shares, but several things can go wrong with this baseline: once the third party receives the labs' data, they may leak the data to others, without the labs' approval; the third party may release fake statistics to the researcher; the third party may release the statistics to the researcher, without checking that it is within the accepted range. In terms of the model, all of these are \textit{unapproved transitions} that, once happened, can lead to agents' constraint states. Yet, on a purely technological level, the agents have no way of preventing these from happening. 

Data Station provides a mechanism to execute any share suggested by an agent, while preventing unapproved transitions \notera{illustrate in the context of a share what are unapproved transitions, e.g., an attacker adds itself as agents, or an attacker changes the input data in a share, or the function, ...}. Crucially, it acts as a \textbf{trustworthy data escrow} (as opposed to a trusted third party), to which the agents delegate their computation of $f(P)$. To execute any share, Data Station first gets the content of the data elements in $P$, using their \textit{type} and \textit{access\_param}, then runs the template function using $P$ and the parameters supplied by some destination agent. The challenge is in ensuring that only approved transitions can happen in this process. Note that another baseline that can execute any shares while only allowing approved transitions is MPC. As we show in Section \ref{sec:evaluation}, Data Station outperforms MPC by orders of magnitudes.

We now make Data Station's security guarantees precise by presenting its threat model.

\mypar{Threat Model} \notera{this first paragraph is not a threat model. The threat model is independent on data station or any other solution} Data Station stores information about agents, data elements, and policies in a database, and stores data elements uploaded by agents on disk. Agents execute shares on Data Station, specified by $f$ (a template function and its parameters) and $P$ (a set of data elements). The expected transition from executing this share is $f(P)$ becomes part of $a_i$'s $D_i$. 

Data Station protects against an adversary who gains access to Data Station infrastructure and can read disk and memory contents. In particular, Data Station ensures that at all times no information about agents, data elements, or policies in their plaintext will ever become accessible to the adversary, 
% 1) following the execution of any share, $f(P)$ and only $f(P)$ become accessible to the destination agent, and 2) no information about agents, data elements, or policies in their plaintext will ever become accessible to the adversary, 
hence preventing unapproved transitions. Denial-of-service attacks are out of the scope of this paper.

\subsubsection{Support for Data Station's Trustworthiness}

\notera{too long. rewrite from scratch summarizing the key points that address what the threat model says. (hint: make sure the threat model makes sense)}

To meet the trustworthiness requirements, Data Station ensures that all data is encrypted end-to-end, from data transfer, to disk storage, to in memory during processing, by leveraging cryptographic protocols and hardware-isolated virtual machines (VMs). 

\mypar{Data Transfer to Disk Storage} Every data element that is uploaded by an agent and stored on Data Station is encrypted with the agent’s specific symmetric key. It is transmitted to Data Station over a secure channel with TLS. Once in Data Station, all data elements remain encrypted at rest.

\mypar{Data In Memory} We give a primer to hardware-isolated VM technology, and in particular, AMD's SEV \cite{kaplan2016amd}. We then explain in details how Data Station leverages SEV, along with a suite of other techniques, to protect data in memory.

Hardware isolated VMs, such as SEV, leverages specially-built hardware to isolate virtual machines to protect data leakage from even privileged users of the system. It guarantees the confidentiality of the application running inside by encrypting all of the OS’s writes to memory. Unauthorized users cannot read data in plaintext, i.e., dumping the memory contents of the process (e.g., cat /proc/[pid]/maps) will show only ciphertext. Agents only need to trust that AMD's hardware is implemented correctly, and the OS image implements SEV correctly.

Since all data elements uploaded to Data Station are encrypted, Data Station needs to decrypt them for processing. To this end, Data Station stores the symmetric keys used by agents to encrypt the DEs. To protect these keys, they are stored in a volatile key manager that resides in-memory. This ensures that all keys are encrypted while Data Station is running. If Data Station restarts (e.g., failure, maintenance), the keys will vanish from the key manager. Data
Station relies on agents re-sending their encryption keys to recover
the keys when necessary.

To compute $f(P)$, Data Station first decrypts all data elements in $P$ in memory using the symmetric keys shared by the source agents. Because memory in SEV is encrypted, both the data element and the keys remain protected from the adversary. After computing $f(P)$, Data Station first encrypts it with the destination agent's symmetric key before transmitting it. 

We explained in Section \ref{subsec:ds_abstractions} that agents write a template function in a high-level language. To allow agents to write functions as they would normally do, while ensuring all data elements on disk are encrypted, Data Station implements an Interceptor middelware using FUSE \cite{}, with the libfuse userspace library used to create file systems in userspace. The Interceptor mounts Data Station’s storage to a specified mountpoint. It intercepts all I/O calls from the a share's execution to storage. Whenever a template function invokes a read operation, the Interceptor decrypts the data on-demand; analogously, it encrypts writes using the destination agent’s symmetric key. 

In addition to protecting the content of data elements, Data Station also ensures that information about agents, data elements, and policies never becomes accessible to an adversary. To achieve this, Data Station creates an in-memory database, which is encrypted by SEV. The challenge is how to deal with reboots of Data Station. To address this, Data Station uses an encrypted writeahead log (EWAL). All updates to the database are first stored encrypted in the EWAL. The entries are encrypted by using the symmetric key of the agent who generated the update, and stored along with the ID of the agent. After restarting, the database can be recovered from the log, as in the traditional recovery protocols of relational databases. To deal with a growing EWAL, the database can be checkpointed to disk periodically.

\notera{these 3 named paragraphs deserve a subsection, as they are about trust and not about how the escrow works}

\mypar{Trusting Template Functions} Without all approval agents approving a share, a share cannot be executed. Yet, it is still up to the approval agents to trust that the template functions are implemented as expected. Data Station adds another layer of security, by creating a "jailed" execution environment for the execution of template functions in shares. The execution environment is implemented as a containerized application that reads the template with its parameters, and runs it. We implement the jail environment to only have access to the relevant $P$; hence, we ensure it is impossible for the template function to access data elements outside of $P$, which could lead to unapproved transitions otherwise. 

\mypar{Trusting Data Station's Implementation} After trusting that Data Station is implemented correctly, and can prevent unapproved transitions from happening, agents may still want to verify that the infrastructure running Data Station has SEV enabled, and is indeed Data Station, not some modified version with injected backdoor. To this end, AMD's hardware allows agents to use remote attestation. This permits agents requesting a report from the node that contains unique identifying information, which provides proof that the node is running Data Station with a correct implementation.

\mypar{Trusting SEV} As the current implementation of Data Station uses SEV to protect data in memory, agents need to trust that AMD’s hardware is correctly implemented and that the OS image implements SEV correctly. This means that our system inherits any vulnerabilities \cite{cohen_technical_2022, li2019exploiting, li2022systematic, li2021crossline, li2021cipherleaks, qin2023protecting, li2021tlb} of the underlying SEV implementation. We would like to notes that Data Station depends on the \textbf{idea} of a hardware-isolated VM, but not any particular implementation, analogous to that the idea of MPC prevents unapproved transitions, but an actual software built using MPC may contain implementation specific vulnerabilities. Thus, accounting for SEV's implementation-specific vulnerabilities is out of the scope of this paper, as these bugs that AMD is actively working to mitigate is independent of the ideas presented in this paper. 



















% An agent writes an EPF program. Upon initialization of Data Station, DS instance also takes in an EPF program. \steven{do we want to say what the EPF program is, a python file?}

% \notera{explain how agents discover what functions are included in the EPF, and how they actually call them}

% There are three endpoints from the server that the agents can call: create\_user, show\_api, and call\_api. \steven{explain what each of these do. show\_api should just lists all the callable apis, as defined by the EPF. Maybe we will have another thing from EscrowAPI that shows the code?}.

% \notera{explain how an interaction among agents could go, and how a "share instance" is set and distributed?}

% Agent creates share, then they’re ACKed or not. Another agent suggests a new share, and then that’s ACKed or not. If CS is not too restrictive, there might be a chance all agents within share will ACK. Then the function is run. 

% \notera{so we are moving the SQL sharing (section 5) here? if so, then we should call this differently. And say, this is an EPF to solve the first stage of the worklow (section 2.1) and help people integrate data.}

% \notechz{Where does trustworthiness go?}

% \notera{end - to integrate}

% \notera{go over an example, briefly, end to end, intertwining the guarantees the escrow provides}

% \notera{explain how an operator could write policies that cannot be circumvented, i.e., to regulate the sharing process}

% \notera{explain "what happens in the escrow stays in the escrow" point to the auditability guarantee and explain why it's important}

% \notera{1. we need to explain agent, policy (important as a contract is a collection of policies), data element, function. 2. then the promise. 3. then say a bit about how the promise is met. 4. then we need to talk about how else (in addition than an escrow) could this whole thing be implemented -> we want to carefully separate what is escrow-specific than what could be implemented on an escrow but does not need to.}

% The EPF defines a \textit{subset} of functions that can possibly be run on data elements. While this somewhat goes against requirement (2), the ability for an agent to openly suggest any function in a share would be impractical; instead, when agents register on Data Station with a specific EPF, they are implicitly allowing only the functionality defined by the EPF. Restricting functionality may be important for scenarios with strict privacy requirements.

% We implement the EPF using Python, but it can be easily extensible to other languages.

% Here is an example of template, written in Python, that 

% \begin{lstlisting}[language=Python]
% def join_tables(attr_left_table, attr_right_table):
%     ...
% \end{lstlisting}

% \begin{myitemize}
%     \item \mypar{Trustworthy} Computation will only run on agent's data upon joint approval of a share. Without an approved share, agents' data will not be visible to anyone, in which case data owners can think of the escrow as an extension to their own infrastructure.
%     \item \mypar{Auditable} Many data release constraints in sharing scenarios involve regulatory and compliance requirements. For example, it may be required that all computation that takes place on the platform needs to be transparent so third-party auditors can audit the sharing agents, otherwise the data cannot be released. The escrow tracks all computation that takes place, and has the ability to make any computation public upon requests.
% \end{myitemize}

% In our model, unintentional data leakage never occurs if unapproved access transitions never occur. For example, a malicious agent such as a hacker may be able to steal data from a poorly secured storage infrastructure, which is an access transition that was never approved. Hence, we build our system around \textit{preventing unapproved transitions}, addressing requirement (1). As a note, we do not consider an attacker obtaining access to encrypted ciphertext as a transition; although they have access to additional data, it is infeasible to obtain the raw data from just ciphertext. We first present a threat model to 

% Hardware-isolated virtual machines are designed to create an isolated execution environment around a VM to minimize the set of all hardware, firmware, and software that agents need to trust to only two components: the vendor hardware and firmware, and the operating system image running in the VM. All other components are untrusted, including the BIOS, hypervisor, other images (in the case of multi-tenant cloud scenarios), and external PCI devices. Examples of these hardware-isolated VMs include AMD's SEV \cite{kaplan2016amd}, Arm's CCA \cite{arm_cca}, and Intel's TDX \cite{intel_intel_2023}. In this paper, we choose to use SEV since, as of May 2023, it is the only commercially available technology with the security guarantees that fit Data Station.

% SEV creates this isolated environment by encrypting all of the OS's writes to memory. Unauthorized users (including by the hypervisor in cloud contexts) cannot read data in plaintext, i.e., dumping the memory contents of the process (e.g., cat /proc/[pid]/maps) will show only cyphertext. Hence a transition here cannot occur.

% We now explain how Data Station is provisioned, from setting up Data Station to the first time a share is approved. At time 0, a developer writes an EPF. A Data Station instance is launched on SEV as a server, along with an EPF program. Agents can attest that Data Station is running on the correct machine, and attest that Data Station's implementation is as expected.

% Once agents trust the Data Station instance is running as expected, they can choose to register as an agent on that instance. Joining the instance running a particular EPF implies that the agent has chosen to become part of the data sharing process, has agreed to the functionalities of manipulating shares and data elements, and are okay with the templates that may be part of shares to be suggested regarding their data elements.

% An agent interacts with the Data Station server by calling one of three APIs: register\_agent, show\_api, or call\_api.
% \begin{myitemize}
%     \item \mypar{register\_agent} Agents call this to register themselves, by specifying a username and password.
%     \item \mypar{show\_api} Agents call this to show all functions tagged with @api\_endpoints.
%     \item \mypar{call\_api} Agents call this to run an API Endpoint, including both template functions and non-template functions.
% \end{myitemize}



==> old/escrow_old2.tex <==
\section{Data Sharing System}

% Data sharing is a process comprised of multiple heterogeneous scenarios 


Data sharing is a process comprised of multiple heterogeneous scenarios, and in this section we describe how this thought process influences design decisions for our data sharing system, Data Station, to support these scenarios through transitions specified by Shares. Our system allows agents to work toward the  resolution of the \textbf{Preparation} and \textbf{Execution} challenges through the Share Abstraction while remaining within the \textbf{Compliance} needs of the agents, assuming agents have the \textbf{Incentives} to share. In Section 4.1 we describe an overview of our system and the requirements for a data sharing system. Section 4.2 details the Data Station as a Share abstraction-based system in detail, and how our system allows for customization for varying sharing scenarios to resolve such preparation and execution challenges. Section 4.3 describes how our system's security only allows transitions approved through shares to occur, which aids in compliance.

\subsection{Architecture Overview}

\label{subsec:overview}

\begin{figure}%
    \centering
    \includegraphics[width=\columnwidth]{figures/ds_overview.png}
    \caption{Data Station Overview}%
    \label{fig:overview}%
\end{figure}

\notechz{Why this thing solves the problems that we have. Also the figure is an overview of an escrow}

\notechz{What is the system goal and how does it work?}

\notechz{If you only have the share abstraction, how can we operationalize that? What is the most basic implementation for the share abstraction? Why did we make the design decisions for this? Why can't we just have lawyers implement the Share, etc.? Why would I implement the share abstraction this way?}

An overview of Data Station infrastructure is shown in Figure \ref{fig:overview}.
\steven{I don't think we want to talk about EPF this early. In 4.1 we want to describe the system using terms everyone can udnerstand. We likely want to start by talking about what agents want to do, what functionalities should be there to support what they want to do, without using any DS specific terminologies. With the way it is written now, it is still bottom-up. I don't see where this is going.}

We let agents tailor an instance of Data Station to support an \textit{entire} data sharing process, from an initial state to a goal state, with an Escrow Programming Framework (EPF). An EPF is written to fit a data sharing process. A developer is an agent, a third party, or anyone with incentive to help drive a sharing process, that writes an EPF. The EPF provides two features to customize for a process: 1) it allows custom-written logic that occurs on top of the Sharing API (\textbf{API Endpoints}); and 2) it allows for custom-written functions that represent $f$ in the model that to be used by Shares (\textbf{Endpoint Functions}). Once an EPF is loaded into Data Station, the API Endpoints are exposed to all agents for them to call, and the Endpoint Functions are registered as all of the possible functions that shares can include when suggested. 

This system builds a workflow for sharing data using Data Station that works toward solving the \textbf{Preparation} and \textbf{Execution} problems of data sharing. We start with an agent that would like to commence a data sharing process. They choose an EPF or write one themselves, and load it into a server hosting an instance of Data Station. We assume agents have the \textbf{incentive} to share when they utilize some discovery process such as a data marketplace or data discovery system and register themselves to Data Station. The server now exposes the API Endpoints of the EPF to these agents. They can see the implementation of the API Endpoints with \textit{show\_function()}, and determine if the customized logic in the API Endpoints and Endpoint Functions suits their sharing scenarios. If so, they can subsequently run \textit{call\_function()} to execute an API Endpoint. Calling API Endpoints multiple times (that call the Sharing API to manipulate data elements and shares), agents communicate and work towards preparing then executing transitions through shares to work toward their goal.

If transitions only occur through shares, relevant agents are cognizant of all transitions relevant to them so they can more easily stay within \textbf{compliance} rules, and auditors can more easily ensure compliance by only having to check the logs of an executed share. In order to only allow approved transitions by Shares to occur, throughout this entire process Data Station leverages cryptographic techniques and hardware-isolated virtual machines to ensure data is encrypted end-to-end, starting from its registration.

To support this share-based workflow, we enumerate the following requirements for a system whose goal is to facilitate an entire process of data sharing.

\begin{myenumerate}
    \item[R1] \textbf{Implement the share abstraction, and support the suggestion and approval of any number of shares, for a wide range of possible shares.} Multiple shares need to be created and executed in a data sharing process. The system needs to allow agents to suggest and approve any number of shares. Moreover, agents may want to execute shares with arbitrary functions and constraints. The system should be flexible enough to support any specifications of the agents, data elements, and functions that define a share. 
    \item[R2] \textbf{Support the execution of suggested shares.} In addition to allowing agents to specify the shares, the system should provide mechanisms to actually execute the shares, i.e. computing $f(P)$. \notera{vague} \notechz{idk what exactly to say here. Steven?}
    \item[R3] \textbf{Ensure all transitions only occur through approved shares.} This helps agents stay compliant. Unexpected transitions such as an attacker gaining access to data that is stored on disk, compromising data in transit, or reading data in-memory during the execution of share, should be protected against.
    \item[R4] \textbf{Meet all requirements above efficiently.} Without reasonable runtime, executing numerous shares to work towards $GS$ will take enough time to discourage sharing.
\end{myenumerate}


\subsection{Escrow API and Escrow Programming Framework}

Data Station provides a native set of APIs for the Escrow Programming Framework to call, which we call the Escrow APIs. Developers utilize two kinds of these APIs when writing API Endpoints: the Sharing APIs, which are implemented as described in \ref{subsec:api}, and the Accessor APIs, which aid in retrieving the agents and data elements for specifying shares. When developers write Endpoint Functions, they call a separate set of APIs to access data elements as they execute.

This set of Escrow APIs are subsequently utilized by API Endpoints and Endpoint Functions.

\subsubsection{Escrow APIs}

Here we describe the APIs necessary to support API Endpoints and Endpoint Functions.

\mypar{Backend for Sharing APIs} API Endpoints call the Sharing APIs to interface with shares, agents, and data elements in Data Station. These Sharing APIs are implemented based on Section \ref{subsec:api} and can register agents and data elements; and suggest, approve, and execute shares. Functions are registered via the EPF. Data Station contains a database that has a table for agents, data elements, and shares. When agents are registered, they input their username and password, are assigned a unique ID, and mark if they are \textit{discoverable} (can be found by Accessor APIs); they are then added to the agent table.

When a data element is registered it is also assigned a unique ID and can be discoverable. Data Station also requires two additional attributes from a data element when it is registered: \textit{type} and \textit{access\_parameters}. These attributes are for capturing heterogeneity of data element types. For example, a relational table stored in CSV can have type "csv", and access\_parameter being the name of the file. A relational table stored on some open data repository can have type "open data", and access\_parameter being a JSON object containing the API key and endpoint from which the data can be retrieved. These two parameters allow Endpoint Functions to customizably access heterogeneous data elements.

The table for Shares consists of a unique ID column along with the four parameters of $A_{\text{ack}}$, data elements, Endpoint Function, and $A_{\text{ack}}$, and is populated when a share is created. This table is also referenced when \textit{show\_share} for a specific share's ID is called. Additionally, another table with columns for $\langle$ Share ID, Agent ID, Approved $\rangle$ represents the $M$ for a share, and the corresponding rows in this table are also added when the share is created. When a Share is executed, this table is referenced; only if all approval agents have approved will the Share execute. Data Station automatically includes all source agents as part of $A_{\text{ack}}$, but agents can add additional approval agents if they desire. These additional agents can be found by using the Accessor APIs. \notechz{make more accurate}

\mypar{Accessor APIs} In some cases, the agent creating a share does not know a priori the agents and data elements that help them achieve their goal. Yet, when a share is specified, it needs to include the complete set of data elements, approval agents, and destination agents. On the other hand, agents may want themselves and their data elements to be discoverable so they can help themselves and other agents to achieve their goals. These APIs reference the tables within the Database and returns discoverable and permitted rows. The API \textit{list\_discoverable\_agents} returns the IDs of agents that are marked discoverable, and likewise \textit{list\_discoverable\_des} returns the IDs of data elements that are marked discoverable.

\mypar{Endpoint Function APIs} These APIs are used to access data elements within an Endpoint Function. The first of these is \textit{get\_de\_by\_id()}, which returns a single data element specified by an ID, if the data element is in P. This data element access the raw data by referring to the \textit{type} and \textit{access\_parameters} fields from when the data element was registered, and behaves accordingly. The other API is \textit{get\_all\_accessible\_des()}, which returns all data elements in $P$ by ID.

Escrow APIs provide the default functionalities for interaction with Data Station, but they are not customizable to a specific process. We introduce the EPF as a layer over this Escrow API that can be written in any way.

\subsubsection{Escrow Programming Framework} An EPF program is a program acting as a customizable layer built on top of the Escrow API, written uniquely for a data sharing process. 

==> old/introduction_old.tex <==
\section{Introduction}
\label{sec:introduction}

\notechz{Motivation for the paper, Convince people that there is a Problem, summarize the Contribution, show people that we can and have evaluated our solution}

Sharing data increases and distributes its value. Oftentimes, groups want to band together and share their data to participate in collaborative data sharing, where all participants have the drive to participate and take action to share data. Hospitals, researchers, chemical companies, and marketers, along with numerous others, have recognized that obtaining and utilizing data relevant to them brings countless benefits such as improved patient care, better products, or better business strategies. Yet, even when these groups have the desire to come together and share, they still find themselves encountering a number of common problems that preclude sharing. Consider the following example.

\begin{exmp}
\label{ex:example}
A researcher contacts three chemical labs, who each holds data about some chemical compounds. The researcher wishes to obtain aggregate statistics about a particular group of compounds, computed from the joint data held by the three labs, and release the statistics to the public. The labs agree to the researcher’s request, but only agrees to share the statistics, not the raw data. Furthermore, the result can only be shared with the researcher if the statistics fall within a certain range. (e.g. the maximum LD50, a measure of the toxicity of chemical compounds, is below some threshold). The researcher agrees to this. The labs use some technology to compute the statistics (e.g. using secure multi-party computation, delegating the computation to a trusted third party, etc.), checks that the computed results are within the allowed range, and proceeds to share the result with the researcher. The researcher then releases the result to the public.
\end{exmp}

\notechz{There are a ton of ways to solve this problem. What is hard about this example today?}

\notechz{A concrete challenge is helping chemical company and researcher to share this data; but these challenges are getting in their way - that's why people should care}
Unless the following problems are resolved, no sharing occurs:
\begin{myitemize}
    \item First, while they desire to share, not every party is hoping to obtain the same shared data; only if data is relevant to the party will they participate. In Example \ref{ex:example}, the researcher does not want to use a lab's data if it is irrelevant to the aggregate statistic.

    \item Second, parties are usually not willing to share all of their data, but can share either a subset or a transformation on it, and they need to clearly define and execute these transformations. In Example \ref{ex:example} the labs only share data if the statistics fall within a certain range, and the aggregate, rather than raw, data is shared.

    \item Third, data is almost never in the same format, schema, or location; data is heterogeneous and this poses a technical challenge that can prevent sharing. In Example \ref{ex:example} the chemical labs' data are potentially stored differently, and data integration techniques may be used through multi-party computation or a trusted third party before the aggregate statistic can be computed.

    \item Fourth, any sharing technology must be secure enough for the parties to use it. The labs in Example \ref{ex:example} would more likely trust secure multi-party computation rather than a trusted third party.
\end{myitemize}


These problems present to every scenario uniquely. Collaboratively sharing data means solving each of these problems for a certain scenario, and hence it is nearly impossible to solve all three of these problems in a single sharing step or computation \notechz{why is it impossible? why is thinking about the process a good thing?}; much more data besides the end result must be communicated and shared. Therefore we think of every data sharing scenario as a \textbf{process} that is unique and must be tailored to the specific scenario at hand.

Specifically, this process is a series of steps. For each step, data is shared to work towards sharing relevant data or solving one of these three problems. Current technologies attempt to resolve only one of these problems, such as multiparty computation for the second problem or data integration for the third problem. While it is possible to use a different technology for resolving each problem, the current technologies solve much too specific problems. Because data sharing is so variable, it is many times the case where, for example, a specific integration technique will not work and a shift to another technology will be necessary. This greatly increases the overhead of sharing, especially when considering security and technical costs. There is no unified system that gives the flexibility and efficiency required to support the numerous technologies and techniques to complete the entire data sharing process on one system. Having this flexibility has the added benefit of allowing for a wide range of sharing scenarios.




\notechz{Data integration within the example as well?}

\notechz{What is the problem?}
The problem is data sharing's own heterogeneity. Every party wants a different thing from sharing data, and every party offers a different thing: they want different data, they want different computation on data. Parties can offer only some data.
The problem is that there are a lot of problems when sharing data. 
Data sharing is a communication-heavy problem.

Our contributions in this paper are:
\begin{itemize}
    \item a model for data sharing
    \item the share abstraction
    \item a data sharing escrow
    \item qualitative usage scenario and quantitative evaluation
\end{itemize}

% \begin{figure}%
%     \centering
%     \includegraphics[width=\columnwidth]{figures/data_sharing_intro.pdf}
%     \caption{How do agents reach the point where all have agreed on how the data will be shared and with whom?}%
%     \label{fig:data_sharing_intro}%
% \end{figure}

% However, even if people want to share data, there exists barriers preventing them from sharing. For example, suppose there are $n$ hospitals, each with some data. They want to run analytics on their joint data, such as studying the effect of a drug on patients. Patient privacy protection laws like HIPAA and each hospital impose constraints on what data can be released, so the hospitals cannot share data with each other directly. It is therefore harder to know whether other hospitals even have data about patients who have received the drug. In addition, each of their data is semantically heterogeneous: they have different schemas, they represent dates in different formats, etc. All these issues can prevent sharing from happening.

% What is hard about helping people achieve their goal, and why is it hard?
% \begin{itemize}
%     \item All data has unique constraints on release. Achieving the goal while abiding by the constraints of all agents' data is hard. (can point to real-life examples of constraints on data release)
%     \item Every agent has requisites on data. Communicating and resolving these requisites can be difficult (we can point to private data integration)
%     \item An ideal mechanism can help agents achieve their goal efficiently while abiding by the constraints of all agents. However, existing work are either inefficient, and/or target a narrow set of constraints, or does not exist for some configurations of sharing scenarios.
% \end{itemize}

==> old/model_old.tex <==
\section{The Data Sharing Model}
\label{sec:model}

Data sharing requires addressing a number of interconnected but otherwise independent problems. In this section, we give intuition to these problems in ~\ref{subsec:prelims}, present a model that delineates data sharing as a process in \ref{subsec:model}, and give examples to illustrate how most real-life data sharing scenarios can be represented using our model in ~\ref{subsec:scenarios}. 

\subsection{Preliminaries}
\label{subsec:prelims}
A prerequisite for data sharing is that a set of entities--such as companies, research labs, or individuals--agree to collaborate and share data with each other. Consider the following example:

\begin{exmp}
\label{ex:example}
A researcher contacts three chemical labs, who each holds data about some chemical compounds. The researcher wishes to obtain aggregate statistics about a particular group of compounds, computed from the joint data held by the three labs, and release the statistics to the public. The labs agree to the researcher’s request, but only agrees to share the statistics, not the raw data. Furthermore, the result can only be shared with the researcher if the statistics fall within a certain range. (e.g. the maximum LD50, a measure of the toxicity of chemical compounds, is below some threshold). The researcher agrees to this. The labs use some technology to compute the statistics (e.g. using secure multi-party computation, delegating the computation to a trusted third party, etc.), checks that the computed results are within the allowed range, and proceeds to share the result with the researcher. The researcher then releases the result to the public.
\end{exmp}

We start by introducing terminologies to discuss Example \ref{ex:example} in detail.

\begin{definition}[Agent]
\label{def:agent}
An agent is an entity with the incentive to participate in sharing data.
\end{definition}

Depending on the context, many types of agents exist, including data owners \cite{syft_2023}, data providers \cite{nguyen2023blockchain, databricks_2023}, data consumers \cite{databricks_2023}, data scientists \cite{syft_2023}, or data requesters \cite{nguyen2023blockchain}. Example \ref{ex:example}'s agents are the researcher, the labs, and the public. Agents can be incentivized to share data for various reasons, such as monetary compensation, or hope to obtain value from the additional data.

In order for data sharing to happen, at least some data is shared between the agents. Naturally, data can be stored in a wide array of formats. The labs can have chemical data as relations in a database, as CSV files, or as images, all of which we call a \textbf{data element}. An agent has access to a set of data elements.

\begin{definition}[Data Element]
\label{def:dataelement}
A data element represents a logical grouping of data that an agent has access to.
\end{definition}

In Example \ref{ex:example}, only the labs have access to relevant data elements at first. The researcher wants to obtain some aggregated statistics on the labs' joint data. The labs are incentivized to help the researcher to achieve this--for example, they may see this as a good act for the public. However, in a data sharing process, agents are also subject to constraints. For example, the labs cannot share the raw data with the researcher, potentially due to regulations.

These agents share their data to act towards their incentives in a series of steps, given their constraints. First, the researcher asks for the labs for the statistics. Upon receiving the request, the labs consider the following factors: with whom is the data shared (the researcher), what data elements are involved (data about chemical compounds), and what transformation should be applied on the data element before it is shared (the aggregates). After considering these factors, the labs agree to the proposal. They calculate the aggregate statistics using some technology, check that the results meet their constraints, and share the result with the researcher. Finally, the researcher releases the result to the public. Once this final step finishes, all agents are satisfied with the data elements they have access to, completing the sharing process.

To our best knowledge, there is no model to precisely describe the entire \textbf{data sharing process}, as illustrated in this example. We now present a model that formally explains what data sharing means in terms of a process, and introduce key abstractions to model the when, what, why, how, and with whom data is shared.

\subsection{Model}
\label{subsec:model}

The data sharing model that we propose envisions data sharing as a process. We first define \textbf{data sharing states}, which describe a snapshot of agents and the data element they have access to at a moment during the data sharing process. 

\subsubsection{States}

\begin{definition}[Data Sharing State]
\label{def:state}

A data sharing state (state) is a pair $\langle\mathbb{A},\mathbb{D}\rangle$. $\mathbb{A}$ is a set of $m$ agents $a_1\ldots a_m$. Each agent $a_i$ has access to a set of $k_i$ data elements $D_i = \{d^i_1, d^i_2, \ldots ,d^i_{k_i}\}$, with $\mathbb{D} = \{D_1\ldots D_m\}$. 

% has a mapping from $a_i$ (i.e. $h_{\text{map}}(a_i) = D_i$).
\end{definition}

After agreeing to share, the involved agents find themselves in an initial state $\langle\mathbb{A}_0, \mathbb{D}_0\rangle$. In Example \ref{ex:example}'s initial state, all agents' $D_i$ is the empty set, except for the labs. These agents want to get to the state where the researcher and the public have access to a statistic on the chemical data. The state agents want to get to is denoted by \textbf{goal state}, which is what drives sharing (explaining \textbf{why} agents want to share data).

\begin{definition}[Goal States]
    Agent $a_i$ acts on their incentive to participate in data sharing by working toward any state in a set of states $GS_i$.
\end{definition}

For data sharing to meet all agents' goals, there exists a \textit{set of common goal states} $GS$:

\[GS = GS_1 \cap GS_2 \cap \cdots \cap GS_m \]

Once the agents reach a state in $GS$, the sharing completes and can terminate. The final state in Example \ref{ex:example} is a goal state because all agents' are satisfied with the data element they have access to. 

% Agents may see overlapping goal states because of external incentives, such as a regulation or a law, or because of internal incentives, such as the prospect of deriving value from sharing.

On the other hand, agents may have data they do not share in the sharing process for various reasons, such as regulations or preference. In Example \ref{ex:example}, the labs will not share their raw data, and will only share aggregate statistics within a certain range. States that agents do not want to get to are denoted by \textbf{constraint states}.

\begin{definition}[Constraint States]
    An agent $A_k$ has a set $CS_k$ of constraint states into which they will refuse to transition.
\end{definition}

Agents may have arbitrary constraint states, such as all states in which their plaintext data is accessible by any other agent. Any state $S$ must stay within the complement of the union of all agents' constraint states, which we call the \textit{total constraint set} $CS$.

\[S \notin CS_1 \cup CS_2 \cup \cdots \cup CS_m = CS \]

If an agent finds themselves in a state within $CS$, at least one agent has not approved of the transition and will, at best, not want to continue sharing. In some cases, goals and constraints are not aligned, thus hampering data sharing. 

\begin{myitemize}
    \item $GS = \emptyset$. In this case, agents' goals are not aligned. 

    \item $GS \subseteq CS$. It impossible for agents to reach a common goal state without the state also being in some agent's constraint state.

    \item $CS$ covers all possible states. Sharing cannot occur, because any state is at least in one agent's constraint states.
\end{myitemize}

Initially, agents may not know each others' goal and constraint states in entirety. It is then up to the agents to figure out how they can reach the goal state by selectively sharing data with each other, while avoiding the constraint states. In doing so, agents make \textbf{transitions} into new states. Transitions describe how one state moves to another.

\subsubsection{Transitions} Throughout a data sharing process that takes multiple steps, agents transition from one state to another as a means to understand each other's constraint and goal states, such that they can work towards $GS$ while avoiding $CS$. Agents may undergo state transitions well before reaching the goal state. For example, when data from multiple sources are desired to be used together, data heterogeneity or data quality issues makes combining the data challenging. To resolve these issues, agents may exchange metadata, share data samples, apply transformations to data such as changing units, all of which lead to a transition to a subsequent state. Eventually, a transition moves the agents to a goal state, or it elucidates that agents' goals and constraints are not aligned.

\begin{definition}[Transition]
\label{def:transition}
A transition is defined as a function $T$ that takes in a state $S$, and outputs another state $S'$.
\end{definition}

Recall that a state is defined by a pair $\langle\mathbb{A},\mathbb{D}\rangle$, describing what agents have access to what data elements. Thus, we define the two possible types of transitions: \textbf{agent transition} and \textbf{data transition}.

\begin{subdefinition}[Agent Transition]
    An agent transition $T_{\text{Agent}}$ is defined by the following parameters: an agent $a_i$, and the agent's corresponding $D_i$. This agent is either removed from or added to $\mathbb{A}$, with $D_i$ removed from or added to $\mathbb{D}$. 
    
    Adding an agent:
    \[ T_{\text{Agent}} (S, a_{\text{i}}, D_{\text{i}}) = S'= \mathbb{A} \cup a_{\text{i}}, \mathbb{D} \cup D_{\text{i}}\]

    Removing an agent:
    \[ T_{\text{Agent}} (S, a_{\text{i}}, D_{\text{i}}) = S'= \mathbb{A} \setminus a_{\text{i}}, \mathbb{D} \setminus D_{\text{i}}\]
\end{subdefinition}

\begin{subdefinition}[Data Transition]
    A data transition $T_{\text{Data}}$ is defined by the following parameters: a set of destination agents $A_{\text{dest}} \subseteq \mathbb{A}$, a set of source data elements $P \subseteq \bigcup^m_{i=1} D_i$, a transformation $f$ to be applied on the data, and a set of approval agents $A_{\text{ack}} \subseteq \mathbb{A}$. Additionally, each approval agent $a_k \in A_{\text{ack}}$ has an approval function $M_k(\cdots) = \{ 0,1\}$. If all $M_k=1$, the transition can take place, and the result of $f(P)$ becomes accessible to every destination agent. Formally,

    \[T_{\text{Data}} (S, A_{\text{dest}}, P, f, A_{\text{ack}}) = S' = \mathbb{A}, \mathbb{D}', \text{where}\]
    
    \[\mathbb{D}' = \begin{cases}

    \{D'_i\}, \text{with } D'_i = 
    \begin{cases} 
      D_i \cup f(P) & a_i \in A_{\text{dest}} \\
      D_i & \text{otherwise}
   \end{cases} & \text{if all } M_k = 1  \\
   
    \mathbb{D} & \text{otherwise}

   \end{cases} 
    \]

       %  if $\exists M_k = 0$

   %  \[\mathbb{D}'=\mathbb{D} \]

   %  Otherwise,

   %  \[\mathbb{D}' = \{D'_i \vert D'_i = 
   %  \begin{cases} 
   %    D_i \cup f(P) & a_i \in A_{\text{dest}} \\
   %    D_i & \text{otherwise}
   % \end{cases}\}
   % \]

\end{subdefinition}

Agent transition describes agents joining in or dropping out from the data sharing process, and does not involve the sharing of data elements between agents on itself. The rest of this section focuses on explaining data transitions, including 1) \textbf{what} data element is shared, 2) \textbf{who} decides to share data with \textbf{whom}, and 3) \textbf{when} can data be shared. Unless otherwise specified, we refer to data transition simply as "transition".

\mypar{What Data Element is Shared} We represent data element shared in a transition with $f(P)$, where $P \subseteq \bigcup^m_{i=1} D_i$ is some subset of all the data elements, and $f$ is a transformation to be applied on $P$ before it is shared. $f$ is general, and can represent any transformation on the data, such as an aggregate query, a machine learning model trained on $P$, or the identity function, in which case the original data elements are shared.

There are two key points in the definition of a transition. First, every agent's set of data elements $D_i$ is monotonically non-decreasing from each transition. That is, transitioning from state $S = \mathbb{A},\mathbb{D}$ to $S' = \mathbb{A},\mathbb{D}'$ necessitates $D_i \subseteq D_i' \quad \forall D_i \in \mathbb{D}$. This comes from the \textit{non-rivalry} property of data \cite{jones2020nonrivalry}, which states that usage of data by one agent does not diminish other agents' use of it. Second, in the definition of a transition, the output of $f$ on some existing data elements $P$ is conceptualized as a new data element, i.e. each data element is different, even in the case when $f$ is the identity function. 
% Hence, in every state, $\lvert \bigcup^m_{i=1} D_i  \rvert = \sum^m_{i=1} \lvert D_i \rvert$. 
This is because once a data element is shared, an agent have little means to control what other agents do with shared data element, on a technical level. Anyone with access to a data element can copy it, modify it, or share it with other agents. 

\mypar{Who Decides to Share with Whom} Before a transition takes place, there exists a set of agents who can approve or deny the transition from happening, which we denote as approval agents $A_{\text{ack}}$. Typically, for a given transition, the approval agents is equivalent to the source agents $A_{\text{src}}$, defined as the set of all unique $a_i$, such that $\exists j, d^i_j \in P$. When the labs shares the aggregate statistics with the researcher, the labs are the both the source agents and the approval agents. In addition to the source agents, the approval agents can also include additional agents, such as an external regulator. After a transition takes place, $f(P)$ becomes accessible to a set of destination agents $A_{\text{dest}}$, representing to whom the data is shared with.

\mypar{When Can Data be Shared} For any transition, the approval agents $A_{\text{ack}}$ need to consider a set of factors before deciding to approve or deny the transition, so that the transition does not lead to some constraint state. We represent the agent's constraints with a function $M_k(\cdots) \rightarrow \{0,1\}$ for every agent $a_k \in A_{\text{ack}}$, with $M_k = 1$ represents approval and $M_k=0$ represents denial. A transition can only occur if all $M_k=1$ for every agent $a_k \in A_{\text{ack}}$. The inputs to $M_k$ are the factors that need to be considered for each transition. For the scope of this paper, we consider the following set of factors: the destination agents $A_{\text{dest}}$, the data elements $P$, the function $f$ to be run on $P$, and additionally some constraints on the output of the function, denoted as $g(f(P))$. 

That is, for a given transition $T_{\text{Data}} (S, A_{\text{dest}}, P, f, A_{\text{ack}})$, there exists a function $M_k$ for every agent $a_k\in A_{\text{ack}}$:

\[M_{k} (A_{\text{dest}}, P, f, g(f(P))) \rightarrow \{0,1\} \quad \forall a_i \in A_{\text{ack}}\] 

A transition $T_{\text{Access}} (S, A_{\text{dest}}, P, f, A_{\text{ack}})$ can only happen if 

\[\forall a_k \in A_{\text{ack}} \quad M_k(A_{\text{dest}}, P, f, g(f(P))) = 1\] 

Consider the transition in Example \ref{ex:example}. Before sharing, the labs have considered the destination agent (the researcher), the data to be shared (the labs' chemical data), and the function $f$ (the aggregate), and have no additional constraint on the output of $f$. The labs approve of this transition ($M_H = 1$), and the transition takes place.

We recognize that in reality, agents may consider arbitrary factor in deciding the value for M. For example, an agent may only share a particular data element when the agent is physically present in North America. We chose a set of representative factors, reflecting the \textbf{what data is shared with whom}, for any given transition. As we later show in Section ~\ref{subsec:scenarios}, these factors are general enough to capture a wide range of real-life sharing scenarios.

\begin{figure}%
    \centering
    \includegraphics[width=\columnwidth]{figures/StateDiagram.pdf}
    \caption{Example \ref{ex:example} decomposed into sequential states using the State Transition Model}%
    \label{fig:model_example}%
\end{figure}

\subsubsection{An Example of Applying the Model} We have introduced a model to describe data sharing as a series of state transitions. We now show how Example \ref{ex:example} can be represented by the model. Figure \ref{fig:model_example} translates the steps in Example \ref{ex:example} to a set of states and transitions.

\steven{skip to 2.3: below text needs to be updated}

\begin{myitemize}
    \item \mypar{State S1} The initial state where relevant data elements are only owned by the hospital. 

    \item \mypar{data transition S1 to S2} The destination agent is the Hospital, with transformation $f_{\text{pii}}$ scrubbing PII from $P=d^H_1$. A new dataset $f_{\text{pii}}(d^H_1) = d^H_{\text{pii}}$ is added to $D_H$. Because the agents have agreed to the data sharing contract, all $M_k = 1$ and the transition is completed.

    \item \mypar{State S2} The hospital has access to new data element $d^H_{\text{pii}}$.

    \item \mypar{data transition S2 to S3} The hospital has shared $d^H_{\text{pii}}$ through an identity function to the researcher, creating $d^R_{\text{pii}}$ from $d^H_{\text{pii}}$ and adding it to $D_R$.

    \item \mypar{State S3} The researcher has access to new data element $d^R_{\text{pii}}$.

    \item \mypar{data transition S3 to S4} The researcher has run the aggregate function $f_{\text{agg}}$ on $d^R_{\text{pii}}$, adding $f(d^R_{\text{pii}}) = d^R_{\text{agg}}$ to $D_R$.

    \item \mypar{State S4} The researcher has access to new data element $d^R_{\text{agg}}$.

    \item \mypar{data transition S4 to S5} The researcher has shared the aggregate statistic $d^R_{\text{agg}}$ with the public with an identity function, creating and adding $d^P_{\text{agg}}$ to $D_P$.

    \item \mypar{State S5}The public now has access to new data element $d^P_{\text{agg}}$.
\end{myitemize}

\subsection{Sharing Scenarios}
\label{subsec:scenarios}

We now show how most real-life data sharing scenarios can be captured by our model. We further show that these data sharing scenarios can be categorized by a set of \textit{data sharing patterns}, revealing commonalities between these scenarios. We start by introducing the two characteristics that define a data sharing pattern: the number of source agents, and the \textit{constraint patterns} agents may have for a given transition.

\mypar{Number of source agents} For a given transition, the source agents $A_{\text{src}}$ are all unique $a_i$, such that $\exists j, d^i_j \in P$. The number of source agents is $\lvert A_{\text{src}} \rvert$. Intuitively, $A_{\text{src}}$ is the set of agents whose data need to be accessed in a transition. We consider two cases: \textbf{single-source} ($\lvert A_{\text{src}} \rvert = 1$), and \textbf{multi-source} ($\lvert A_{\text{src}} \rvert > 1$). In the single-source case, only one agent has data to share. In the multi-source case, multiple agents want to share their joint data.

\mypar{Constraint Patterns} Approval agents specify whether they approve or deny a transition by specifying either 0 or 1 for $M$. Based on what factors to M are of interest to the approval agents, we enumerate the following \textit{constraint patterns}:
\begin{myitemize}
    \item Preconditional: Agents have constraints on $A_{\text{dest}}$, $P$ and $f()$, before $f$ even runs (hence preconditional). For example, agents may approve running an aggregate on their data and releasing it to some authorized agents, but revealing the plaintext data, in which case $f()$ is the identity function, is unacceptable. If the number of source agents is one, only that agent needs to approve. Otherwise, all source agents must agree on whether to run the function. 
    \item Postconditional: Agents have constraints on $f(P)$, specified through $g(f(P))$, after $f$ runs (hence postconditional). For example, one agent $a_1$ may ask for a query result on another agent $a_2$'s data, and $a_2$ will only release the result if the output has cardinality larger than some threshold.
    \item Biconditional: Since preconditional and postconditional are not mutually exclusive, agents can have constraints on $A_{\text{dest}}$, $P$, $f()$, and $g(f(P))$, hence biconditional.
    \item Unconditional: Agents unconditionally set $M$ to 1.
\end{myitemize}

A data sharing pattern is defined by a specification of these two characteristics: the number of source agents, and the constraint patterns. Below we give a set of data sharing patterns, and give real-life data sharing scenarios that fall under these patterns. We recognize that real-life data sharing scenarios can be much more nuanced. The scenarios as described below are not meant to replicate real-life data sharing scenarios exactly, but to capture them in sufficient details to illustrate the generality of our model.

\mypar{Single-source, Unconditional} One example is an individual posting data online for the public, such as to twitter or a personal website. The posted data becomes accessible unconditionally to any $A_{\text{dest}}$ that wants it.

\mypar{Single-source, Preconditional} One example is sharing the MIMIC-III health data online\cite{johnson2016mimic}. Only users who have completed a training and signed a user agreement can access the data. Another scenario is Delta Sharing\cite{databricks_2023}, where agents put data in a "Share". To share this data, they add other agents to the "Share", such that all those agents get direct access to all data within the "Share". Agents can also have constraints on both $A_{\text{dest}}$ and $f$. One scenario is an administrator sets up an enterprise-internal Postgres server, and only allows specific users to run specific queries against the database.

\mypar{Multi-source, Unconditional} One example is the national census, in which all citizens' data are unconditionally collected from them, after which some aggregate information are calculated and released back to the public. The number of source agents is equal to the US population. By law, the source agents do not get to choose whether their data is sent to the census or not.

\mypar{Multi-source, Preconditional} One example is the notion of a data federation, as described in \cite{bater2017smcql, bater2020saqe, volgushev2019conclave}. At time 0, it is assumed that a set of agents agree upon a set of SQL queries to run on their joint data, which all share the same schema. The goal is for all of them to get access to the query results. This line of work typically poses the additional constraint that no agents $a_i$ will allow any other agents to access their data $d_i$ in plaintext, that is, $M(*, d_i, f_{\text{identity}}, *) = 0 \; \forall a_i$ at all times. 

\mypar{Multi-source, Biconditional} One example is the collaborative learning platform, as described in \cite{zheng2021cerebro}, which targets the specific use case of training machine learning models. In addition to assuming that all agents have agreed on the model to train, agents can also describe \textit{release policies}, such as only releasing the joint model if its accuracy is higher than some threshold. This is equivalent to the notion of a postconditional constraint ($g(f(P))$). Another example is Snowflake's  data clean room\cite{kaufman_2022}. An agent with data specifies a template SQL query to run. Other agents can submit requests that follow this template that need to be approved by the source agent. The template query can also include relational conditions (e.g. number of unique values in a column $>25$), thus implementing a portion of the postconditional constraints on the query result. 

% \mypar{Notation} We use $*$ as a parameter to M to represent wildcard matching, meaning that agent has no constraint on that parameter when defining their M. We use $I$ to represent the identity function. Sharing $I(d)$ of data element $d$ is equivalent to sharing the original $d$.

% \begin{figure}%
%     \centering
%     \includegraphics[width=\columnwidth]{img/pattern_diagram.pdf}
%     \caption{The Four Constraint Patterns: Preconditional, Postconditional, Biconditional, Unconditional}%
%     \label{fig:pattern_diagram}%
% \end{figure}

% \subsection{Existing Support within the Model}
% \label{subsec:existing}

% \begin{myitemize}
%     \item Allowing conditionals
%     \item If you are to allow conditionals, a clear expression of the transition triple is necessary.
%     \item Running transitions correctly, e.g. a state is transitioned as advertised.
% \end{myitemize}

% In this section we explore existing technologies used to implement transitions. These technologies must ensure that the desired transition is run. \notechz{"Desired" means Aack} For example, a security breach or an incorrectly-run function would lead to an undesirable data transition to $S'' \in CS$. Existing technologies make various attempts at supporting the representation of a transition, enabling patterns, and ensuring these transitions are run correctly. We outline the space of these work in Table \ref{tab:technologies}.

% \steven{I think the table should be improved, in terms of the information we actually include in it. I am just not sure what the changes should be yet.}

% \begin{table*}[]
%     \centering
%     \begin{tabular}{|c||c|c|c|c|}
%         \hline
%         \textbf{Technology} & \textbf{M-N} & \textbf{Preconditional} & \textbf{Postconditional} & \textbf{Possible} $f$ \\
%         \hline
%         \hline
%         Delta Sharing \cite{databricks_2023} & 1-N & Must be Approved to a "Share" & None & Identity Only (Plaintext) \\
%         \hline
%         Google Ads Data Hub \cite{google_2023} & 2-N & None & None & Aggregates Only \\
%         \hline
%         SMCQL \cite{bater2017smcql} & 2-N & Assumed Approval & None & Most SQL Queries \\
%         \hline
%         Conclave \cite{volgushev2019conclave} & 2/3-N & Assumed Approval & None & Conclave's LINQ-like language \\
%         \hline
%         Hu-Fu \cite{tong2022hu} & M-N & Assumed Approval & None & Spatial Queries \\
%         \hline
%         Cerebro \cite{zheng2021cerebro} & M-N & Assumed Approval & Release Policies & Machine Learning Workloads \\
%         \hline
%         Snowflake Cleanroom \cite{kaufman_2022} & M-N & Approval Required & Only SQL Conditions & SQL Templates written by source agent \\
%         \hline

%     \end{tabular}
%     \caption{The Space of Existing Sharing Technologies}
%     \label{tab:technologies}
% \end{table*}

% \begin{myitemize}
%     \item \mypar{Delta Sharing} 
%     \cite{databricks_2023} Databricks' Delta Sharing falls under a 1-N Preconditional pattern. No agent can get access to the data until they are added to a "share", which is effectively an approval method. But, any tables added to the share can be accessed by agents within the share in full plaintext. Hence, Delta Sharing supports only identity functions $f()$.

%     \item \mypar{Google Ads Data Hub} \cite{google_2023} Ads Data Hub is a M-N Unconditional pattern. Any user of Ads Data Hub combines their data with Google's ad data, producing an aggregate function that is released to the user. However, since only aggregate functions are allowed to be run, the possiblities of $f()$ are only aggregates.

%     \item \mypar{Secure Multi-Party Computation Systems (MPC)} MPC is a technology for cryptographically computing and distributing the results of a function within a M-N Preconditional pattern. Many MPC work \cite{bater2017smcql, volgushev2019conclave, tong2022hu, wang2021secure} suggest that some kind of agreement, decided beforehand, on which $f()$ to run on agents' joint data. This agreement assumes away the preconditional pattern. Cerebro also supports the postconditional pattern through \textit{release policies}, such as adding DP noise to output. \cite{zheng2021cerebro}. 
    
%     In theory, MPC can support any $f$. Yet, most current MPC system's implementations targeted at data sharing are restricted in the type of $f$ they support, such as a limited set of relational operators.
    
%     \item \mypar{Snowflake Cleanroom} \cite{kaufman_2022} This is one implementation of a M-N biconditional pattern for relational queries. An agent with data specifies a template SQL query to run, then other agents can submit requests that follow this template that need to be approved by the source agent. The template query can also include relational conditions (e.g. number of unique values in a column $>25$), thus implementing a portion of the postconditions on the query result. The restriction of using template relational queries, as defined by the source agent, restricts the space of $f()$ and the set of possible postconditional patterns.

%     \steven{this is not an existing technology: we move this to later sections}
%     \item \mypar{Trusted Third Party} A trusted third party can be asked to execute any M-N patterns for any constraint pattern. However, this trusted third party may unexpectedly deviate from the protocol to execute the exact transition requested, which means a different transition is executed instead. For example, a trusted third party may leak data while running the computation, transitioning to an undesirable state.
    
% \end{myitemize}


% Existing solutions implement only a specific subset of data sharing patterns. What is needed is a system that reflects data sharing as a process by (1) posing no restriction on the source agents, the destination agents, the type of $f()$ supported, and the set of constraint patterns supported (Section \ref{sec:share}) and (2) allowing an arbitrary number of state transitions until the goal is achieved (Section \ref{sec:escrow}).


==> old/scenario_old.tex <==
\section{Use Case: SQL and Data Integration}
\label{sec:usagescenario}

We now show how agents can use our system in the data sharing process through a usage scenario. The datasets and schema we use are based on the monitor dataset from the DI2KG'20 workshop at VLDB 2020 ~\cite{di2kg}, which is extracted from multiple, real e-commerce websites. The scenario is as follows. Consider 3 websites: eBay, PC Canada, and XPC. Each of them has access to a set of monitor specifications for monitors sold in the past month. Data analysts working for the 3 websites want to run some analysis on their joint data. Since this is real-world data collected by three different websites, their schema is heterogeneous, and the analysts need to go through a series of steps in order to run analysis. This helps us illustrate how our system facilitates the entire data sharing process.

\mypar{Background} The schema for each website's monitor dataset is as follows:
\begin{itemize}
    \item eBay: \textbf{brand, color, microphone, screen type}
    \item PC Canada: \textbf{brand name, speakers, number of speakers, aspect ratio}
    \item XPC: \textbf{product type, builtin speakers, height}
\end{itemize}
These schema are simplified versions of the websites' actual schema in ~\cite{di2kg}, as the actual ones contain more than 100 attributes each. We use the simplified schema for clearer illustration. In reality, before querying the joint data, the analysts from each website may choose to pre-process their data, and keep only a small subset of attributes deemed potentially relevant.

One way in which the analysts can run analysis on joint data is by sending all relevant data to one analyst. Yet, the analysts do not want to do that, as the data contains sale records that are considered sensitive. In fact, the analysts wish to integrate their data such that their query can run successfully, while revealing as little as possible during the process.

\mypar{1. Setting up and Defining EPF} The analysts create an initial EPF, with direct calls to Escrow API for \textit{register\_data()}, \textit{upload\_data()}, \textit{suggest\_share()} and \textit{approve\_share()}. Since the analysts wish to achieve data integration while revealing no more data than necessary, they create the following template functions:
\begin{itemize}
    \item \textit{show\_schema()}, which returns the schema of every data element in $P$.
    \item \textit{show\_intersection\_size(de\_id1, attr1, de\_id2, attr2)}, which takes in the names of two attributes, one from each input data element, and returns the size of their intersection.
    \item \textit{show\_sample(de\_id, size)}, which returns a sample with the specified size for de\_id.
    \item \textit{run\_result\_query(query)}, which takes in a SQL query, and executes on the joint $P$. It first creates a DuckDB relation by unioning all agents' data element together, after resolving the schema heterogeneity, then execute the query on top of the joint relation.
\end{itemize}

The analysts start a server running the Data Station with the above EPF loaded, and register themselves as agents (denoted $a_1$, $a_2$, and $a_3$) of the Data Station. They also register their data elements (denoted $d_1$, $d_2$, and $d_3$) and upload them to the Data Station.

\mypar{2. Sharing Schema} As a starting point, the analysts want to show each other the schema of their data. One of the analysts proposes an initial share by calling \textit{suggest\_share($A_{\text{dest}}$, $P$, show\_schema)}, with $A_{\text{dest}}$ being $a_1, a_2, a_3$, and $P$ being $d_1, d_2, d_3$. Since the EPF uses the default implementation of \textit{suggest\_share}, Data Station automatically populates the owner of the data elements as $A_{\text{ack}}$. All analysts call \textit{approve\_share()}, so that they can access the schema of all the relations. 

After seeing the schema, analysts from PC Canada and XPC realize that the relation from eBay does not seem to have overlapping attributes of interest to them. The two decide to continue sharing only between themselves. In particular, they decide that they want to run a query on their joint data to to get the total count of monitors sold with a built-in speaker. 

\mypar{3. Resolving schema heterogeneity} Analysts from PC Canada and XPC suspect that the attributes \textbf{speakers} and \textbf{builtin speakers} from their respective relations mean the same thing. To make sure of this, one of them calls \textit{suggest\_share()} to suggest the following share:

\[\langle (a_2, a_3), (d_2, d_3), show\_intersection\_size() \rangle\]

The input parameters are $(d_2, \text{speakers}, d_3, \text{builtin speakers})$. However, after approving and running the function, the analysts notice that there is no overlap between the values from these two columns. To investigate the reason, $a_2$ decides to ask $a_3$ for a sample of their data, suggesting a share with \textit{show\_sample} and a size of 50. Yet, $a_3$ thinks the sample size is too large, and would like to keep the revealed sample as small as possible. Thus, $a_3$ does not approve of the share $a_2$ suggests, but suggests another share, also with \textit{show\_sample}, but only a size of 10. $a_3$ then approves of the share, since he is by default $A_\text{ack}$. 

$a_2$ runs this share, and figures that \textbf{speakers} in $d_2$ consists of "Yes" and "No", whereas \textbf{builtin speakers} in $d_3$ consists of "Y" and "N". This data heterogeneity leads to empty column intersection. Thus, $a_2$ applies a transformation to $d_2$ to change all "Yes" and "No" to "Y" and "N". He then registers the updated relation as a new data element $d_4$ with the Data Station.

\begin{figure}%
    \centering
    \includegraphics[width=\columnwidth]{figures/code.png}
    \caption{EPF Code Snippet for run\_actual\_query}%
    \label{fig:model_example}%
\end{figure}

\mypar{4. Actual query execution} At this point, both analysts believe that they have successfully integrated their data, and are ready to execute the query. Figure ~\ref{fig:model_example} shows the code snippet for the implementation of \textit{run\_actual\_query()} in the EPF. It takes in a SQL query string, and a table name string. First, the function gets the id of all the accessible data elements. \textit{assemble\_table\_in\_duckdb} then runs, which is a helper function defined in the EPF that create a table with name \textbf{joint table name} in the DuckDB engine. Lastly, DuckDB executes the query given by the user, and returns the result. Note that this is just one implementation of running a query. If all the schema is known a priori, and the analysts only want to run one specific query, they can directly code the query in the EPF. If the data contains sensitive information, and the analysts want to add differentially private noise to the result, they can use any library they want to add the noise after query result is computed, before returning it. They can also define arbitrary postconditionals, by requiring the query result to only be released after meeting some specified conditions. The flexibility of a template in Data Station enables all these functionalities, thus supporting a wide range of possible transitions. 


==> old/share_old.tex <==
\section{Sharing API}
\label{sec:share}

% \steven{in section 3, people should be thinking about software and APIs, not the mathematical model. We want the share abstraction to fully support section 2. Goal of 3: convincing people that data sharing can be implemented in software, using the share abstraction and the set of APIs we propose}

We have explained data sharing as a series of transitions from one state to another, where agents either reach a common goal state, or realize that no such state exists. We now introduce the \textbf{share abstraction}, and a set of APIs to manipulate the abstraction. Together, they show how a system that supports any data sharing scenarios can be implemented. The abstraction itself and the set of APIs are independent of the underlying technology used for implementation.

\subsection{The Share Abstraction}
\label{subsec:share-def}

In a data sharing process, agents need to precisely communicate the transitions they want to happen. In terms of our model, this means that agents need to be able to specify the \textbf{who} ($A_{\text{ack}}$) decides \textbf{when} ($M$) to share \textbf{what} data ($f(P)$) with \textbf{whom} ($A_{\text{dest}}$). After a transition is specified, $A_{\text{ack}}$ now need to know these attributes that define the transition and then be able to communicate their value of $M$ as 0 or 1.

We propose the \textit{share} abstraction, which enables agents to do the above for any transition.

\begin{definition}[Share]
    A \textit{share} abstraction is a quadruple

    \[\langle A_{\text{dest}}, P, f, A_{\text{ack}} \rangle\]

    with a function $M_{k}(\cdots) \rightarrow \{0,1\}$ for every $a_k \in A_{\text{ack}}$. $A_{\text{dest}}$ represents a set of destination agents, $P$ represents a set of data elements as inputs to $f$, and $f(P)$ is to be shared to all of the destination agents. $A_{\text{ack}}$ is the set of agents who can approve the share with $M_k$. The content of a share is visible to all of $A_{\text{ack}}$.
\end{definition}

Note the similarity between the definition of a share and the definition of a transition. This is no coincidence, as the share abstraction is designed for the specific purpose of allowing agents to communicate transitions. Exactly like a transition, the share specifies a set of data elements, a transformation to be applied on the data elements, the destination agents that receive data, and the agents who can approve of the transition. 

In order for the approval agents to decide on the value for each of their $M$, the content of each share needs to be visible to all agents in $A_{\text{ack}}$. The content of a share includes all the information that captures an agent's preconditional constraints, which are $A_{\text{dest}}$, $f()$, and $P$. For agents' postconditional constraints on $g(f(P))$, those can be built into $f$, because $f$ can be any function. We will give an example of how this is done with an example in ~\ref{subsec:share-pattern}.

A single share specifies to a particular transition. As most data sharing scenarios consist of a series of transitions, we envision data sharing as a continual process of suggesting, showing, approving, and executing shares. We now present a set of APIs to facilitate this process.

\subsection{Sharing API}

A share is specified by a combination of agents, data elements, and functions. These abstractions need to be registered somewhere, so that they can be referred to when specifying shares. To this end, the following set of APIs need to exist:

\myparnoperiod{register\_agent()} This API is used for the registration of agents. An agent should be registered, such that they can be included as part of $A_{\text{ack}}$ or $A_{\text{dest}}$.

\myparnoperiod{register\_data\_element()} This API is used for the registration of data elements $d^i_j$. As explained in Section \ref{sec:model}, data elements can be stored in a wide array of formats and granularity. Hence, the implementation of this API should be able to capture these heterogeneity. Furthermore, each data element $d^i_j$ needs to be associated with a registered agent $a_i$ to reflect that $d^i_j$ is in $a_i$'s $D_i$.

\myparnoperiod{register\_function()} This API is used for the registration of functions $f()$. Functions will be applied on data elements.

Once there exists APIs to register agents, data elements, and functions, agents can now make use of shares. In particular, agents can interact with shares in the following ways: suggesting a new share, showing the content of an existing share, approving an existing share, or executing a share. These lead to the following APIs:

\myparnoperiod{suggest\_share()}  This API creates a new share. The input includes the information needed to create a share: who approves ($A_{\text{ack}}$), what is shared ($f(P)$), and to whom is the data shared ($A_{\text{dest}}$). Typically, $A_{\text{ack}}$ needs to include the source agents of $P$, but others such as auditors or regulators can also be specified. On the implementation side, there needs to be some mechanism of specifying then executing $f$.

\myparnoperiod{show\_share()} This API displays the content of a share. When a share is first suggested, no approval agent in $A_{\text{ack}}$ has approved of the share. An approval agent need to calls this API to know the share's specification, so that they can decide on a value for their $M$.

\myparnoperiod{approve\_share()} An approval agent calls this API to approve a share by setting $M=1$. It is possible that an agent does not approve of a particular share (e.g. $f$ violates the agent's constraint), but still wants to continue the sharing process. In this case, agents may suggest an alternate share.

\myparnoperiod{execute\_share()} A destination agent calls this API to run and get access to $f(P)$. Only when all agents in $A_{\text{ack}}$ have approved of the share can a share be executed.

Together, this set of APIs allows any data sharing scenario to be built on top of it.

\subsection{Example of Using the Share Abstraction}
\label{subsec:share-pattern}

We now give an example of how the share abstraction can be used to implement the sharing scenario in Example \ref{ex:example}. We denote the labs as $\{a_1, a_2, a_3\}$, and the researcher as $a_0$. At time 0, all agents register themselves. In addition, the labs register their data elements.

The researcher initially registers $f_{\text{agg}}$, which directly runs an aggregate query on the input data elements. He then calls \textit{suggest\_share} with 
\[A_{\text{dest}} = \{a_0\}, P = \{d^1, d^2, d^3\}, f_{\text{agg}}, A_{\text{ack}} = \{a_1, a_2, a_3\}\]

Yet, the labs are only willing to share the data, subject to the postconditional constraint that the statistics can only be shared if it falls within a certain range. Thus, instead of approving the original share, they register a new function $f_{\text{modified}}$, which is the same function that the researcher proposes to run, with the exception that the output will be set to NULL if it is not within a range. The labs then suggest the following share instead:
\[A_{\text{dest}} = \{a_0\}, P = \{d^1, d^2, d^3\}, f_{\text{modified}}, A_{\text{ack}} = \{a_1, a_2, a_3\}\]

The labs approve of this share, and the share is ready to be executed by the researcher. In this example, the transition captured by this share falls under the multi-source, biconditional pattern, as multiple source agents' data elements are accessed, and the chemical labs only agree to share the aggregate statistics with the researcher, subject to constraints on the statistics. Being able to support the multi-source, biconditional pattern shows that the share abstraction can support any data sharing patterns, and hence any data sharing scenarios.



==> todo.tex <==
\section{To-do List}

\begin{itemize}
    \item Finish SQL EPF implementation and verify correctness. \steven{part done}
    \item Write section "Introduction" \steven{part done}
    \item Write section "Data Sharing patterns"
    \item Write section "Share abstraction"
    \item Write section "Escrow programming framework
    \item Write section "SQL sharing APIs"
    \item Write section "Related work"
    \item Design experiments for query execution comparisons: what dataset, which benchmarks, which plots, what do the axis represent (need to draw it out on paper) \steven{part done}
    \item Do experiments for query execution comparisons, once the above is done.
    \item Design experiments for micro-benchmarks: local vs remote data access. Requirements are the same as above. \steven{part done}
    \item Do experiments for micro-benchmarks. 
    \item Design "experiments" to evaluate that our system allows people to integrate data with meeting their data release constraints.
    \item Do experiments for the above.
\end{itemize}

\label{sec:todo}
